Scene Transformer: A unified architecture for predicting multiple agent trajectories

Predicting the motion of multiple agents is necessary for planning in dynamic environments. This task is challenging for autonomous driving since agents (e.g. vehicles and pedestrians) and their associated behaviors may be diverse and influence one another. Most prior work have focused on predicting independent futures for each agent based on all past motion, and planning against these independent predictions. However, planning against independent predictions can make it challenging to represent the future interaction possibilities between different agents, leading to sub-optimal planning. In this work, we formulate a model for predicting the behavior of all agents jointly, producing consistent futures that account for interactions between agents. Inspired by recent language modeling approaches, we use a masking strategy as the query to our model, enabling one to invoke a single model to predict agent behavior in many ways, such as potentially conditioned on the goal or full future trajectory of the autonomous vehicle or the behavior of other agents in the environment. Our model architecture employs attention to combine features across road elements, agent interactions, and time steps. We evaluate our approach on autonomous driving datasets for both marginal and joint motion prediction, and achieve state of the art performance across two popular datasets. Through combining a scene-centric approach, agent permutation equivariant model, and a sequence masking strategy, we show that our model can unify a variety of motion prediction tasks from joint motion predictions to conditioned prediction.

==> sections/acknowledgements.tex <==
\subsubsection*{Acknowledgements}
\noindent We thank Dragomir Anguelov, Scott Ettinger, Yuning Chai, Andre Cornman, Rami Al-Rfou, Mark Palatucci, Balakrishnan Varadarajan, Barret Zoph, and Shuyang Cheng for their comments and suggestions. Additionally, we thank the larger Google Brain, Google Perception, and Waymo Applied Research teams for their support.


==> sections/contributions.tex <==
\subsubsection*{Author Contributions}
JN conceived of the modeling approach. JN, VV and BC co-led the project and developed models, infrastructure, experiments, evaluations, and analysis. ZZ developed several architecture innovations that led to notable improvements, and ran many experiments to tune, optimize and improve the model performance. HC developed several modeling and novel data augmentation innovations that led to notable improvements, and ran many experiments to improve model performance. AB ran many experiments to improve the performance of the marginal predictions of the model, and analyzed the relative performance of the marginal and joint prediction model. RR led much of the analysis of the model performance, and investigated the robustness of the model architectures. CL ran experiments to improve the overall performance of the model, and led much of the experiments and analysis on conditional behavior prediction. JL, DW and AV led the experiments focused on goal-directed planning. BS offered much discussion and ideas surrounding behavior prediction, and helped write the paper. ZC helped develop the infrastructure and provided guidance and mentorship. JS helped write the paper, coordinate the project, and provide guidance and mentorship.

==> sections/impact.tex <==
\section*{Broader Impact}

The work presented has the potential to improve the reliability and accuracy of autonomous vehicles. Autonomous vehicles have the potential to provide numerous benefits to society in terms of reduced car accidents due to human error as well as improving the mobility of individuals with disabilities. We note however that the potential benefits from autonomous vehicles do not result directly from the technology, but instead require a continued commitment to an equitable and responsible deployment of such technology.

%{\bf Version 1} The work presented has the potential to improve the reliability and accuracy of autonomous vehicles. Autonomous vehicles have the potential to provide numerous benefits to society in terms of reduced car accidents due to human error as well as improving the mobility of individuals with disabilities. We note however that the potential benefits from autonomous vehicles do not result directly from the technology, but instead require a continued commitment to fairness, social justice and privacy in the deployment of such technology.

%{\bf Version 2} This paper presents a machine learning system for predicting the behavior of agents often encountered in the autonomous vehicle environment, such as pedestrians, vehicles and cyclists \cite{REF:lyftperception2019,sun2020scalability,geiger2013vision}. In addition, this system provides the ability to learn how to navigate an autonomous vehicle through such an environment predicated on the learned interactions with other agents. Although this work motivates our work based on the application of autonomous vehicles, such work may subserve the development of intelligent robotic systems that must predict the behavior of external agents and successfully navigate within this environment.

%Software that governs the actions of autonomous vehicles requires that safety be a critical consideration for judging the efficacy and deployment of such a system \cite{kalra2016driving,koopman2017autonomous}. Two important tasks for autonomous vehicles addressed in this paper include (1) correctly predicting and anticipating the actions of other pedestrians and vehicles and (2) selecting an appropriate route to navigate amongst these other agents in the environment. The degree to which an autonomous vehicle may correctly address these tasks influences the overall safety and efficacy of the system. Thus, the development of such behavior prediction and planning systems is only the initial step, and the true onus of deploying such systems is testing the safety of the vehicle in the real world \cite{norden2019efficient,o2018scalable}. We note that addressing the tasks discussed in this paper do not constitute a fully operational autonomous vehicle, but merely provide one component of such a system. Accordingly, the overall safety profile of a vehicle may be governed and heavily influenced by the efficacy of other systems, e.g. perception systems \cite{geiger2013vision,thrun2006stanley} and the interplay of these systems in the real world environment.

%Serious ethical considerations have been heavily discussed in the public sphere with regard to the deployment of autonomous vehicles. Most notably, the deployment of an autonomuous vehicle generates the potential risk for the loss of human life, and accordingly any decisions about the deployment of this technology needs to weigh multiple factors. Most prominent, many have noted that the number of car accidents due to human drivers, whether due to intoxication, drowsiness or simple human error, result in an inordinate number of premature deaths and is one of the leading causes of premature death in the world \cite{}. Accordingly, many have argued that it would be morally wrong not to deploy autonomous vehicles if they perform statistically better than human drivers \cite{sparrow2017human,kalra2017challenges}. To that end, many firms in the autonomous vehicle industry publish detailed reports about the safety profile of their vehicles \cite{aurora-safety,lyft-safety,waymo-safety}.

%Another dimension of autonomous vehicles technology is consideration of the many data privacy issues that surface in gathering large datasets from the real world to train the resulting machine learning systems \cite{papernot2016towards,horvitz2015data}. First, serious consideration must be warranted to expose, address and resolve potential issues of systemic bias \cite{mitchell2019model}. Second, training machine learning systems based on such datasets need to ensure that private data is not unintentionally leaked. Multiple opportunities are available for addressing these issues including federated learning techniques \cite{mcmahan2017communication} and training models with differential privacy-based mechanisms \cite{dwork2008differential,abadi2016deep}.


==> sections/old/architecture-table-old-old.tex <==
% /cns/oi-d/home/chauffeur/ml/tensorflow/bencaine/babelfish/rs=6.3/ttl=90d/waymo_mod_head_04_29_21.v0/train_train/model_analysis.txt
\begin{table*}[ht]
\small
\centering
\bgroup
\def\arraystretch{1.2}%  1 is the default, change whatever you need
\begin{tabular}{llcccccc}
\toprule
& Input & Operation & Queries & Keys/Values & Across & Atten Matrix & \# Param \\
\midrule
{\bf Encoder} \\
%\midrule
& $[A, T, K]$ & MLP & -- & -- & -- & -- & \todo{?} \\
\\
& $[A, T, D]$ & Transformer & Agents & Agents & Time & $[A, T, T]$ & \todo{?} \\
& $[A, T, D]$ & Transformer & Agents & Agents & Agents & $[T, A, A]$ & \todo{?} \\
\\
& $[A, T, D]$ & Transformer & Agents & Agents & Time & $[A, T, T]$ & \todo{?} \\
& $[A, T, D]$ & Transformer & Agents & Agents & Agents & $[T, A, A]$  &  \todo{?} \\
\\
& $[A, T, D]$ & Transformer & Agents & Agents & Time & $[A, T, T]$ & \todo{?} \\
& $[A, T, D]$ & Transformer & Agents & Agents & Agents & $[T, A, A]$ & \todo{?} \\
\\
& $[A, T, D]$ & Transformer & Agents & Road Graph & Time & $[T, A, G]$ & \todo{?} \\
%$[A, T, D]$ & Transformer & Agents & Road Graph & $[A, G, G]$ &  \todo{?} \\
\\
& $[A, T, D]$ & Transformer & Agents & Agents & Time & $[A, T, T]$ & \todo{?} \\
& $[A, T, D]$ & Transformer & Agents & Agents & Agents & $[T, A, A]$ & \todo{?} \\

\midrule
{\bf Decoder} \\
& $[A, T, D]$ & Tile & -- & -- & -- & -- & 0 \\
& $[F, A, T, D]$ & Concat & -- & -- & -- & -- & 0 \\
& $[F, A, T, D+F]$ & MLP & -- & -- & -- & -- & \todo{?} \\
\\
& $[F, A, T, D]$ & Transformer & Agents & Agents & Time & $[A, T, T]$ & \todo{?} \\
& $[F, A, T, D]$ & Transformer & Agents & Agents & Agents & $[T, A, A]$  &  \todo{?} \\
\\
& $[F, A, T, D]$ & Transformer & Agents & Agents & Time &  $[A, T, T]$ & \todo{?} \\
& $[F, A, T, D]$ & Transformer & Agents & Agents & Agents & $[T, A, A]$  &  \todo{?} \\
\\
& $[F, A, T, D]$ & Transformer & Agents & Agents & Time & $[A, T, T]$ & \todo{?} \\
& $[F, A, T, D]$ & Transformer & Agents & Agents & Agents & $[T, A, A]$  &  \todo{?} \\
\\
& $[F, A, T, D]$ & Transformer & Agents & Agents & Time & $[A, T, T]$ & \todo{?} \\
& $[F, A, T, D]$ & Transformer & Agents & Agents & Agents & $[T, A, A]$  &  \todo{?} \\
\\
& $[F, A, T, 6]$ & MLP & -- & -- & -- &  -- & \todo{?} \\
%\midrule
%{\bf Total} & & & & & & & 15,625,101 \\
\midrule
% https://source.corp.google.com/piper///depot/google3/waymo/shared/brain/behavior_understanding/params/waymo_mod.py;l=254
% /cns/oi-d/home/chauffeur/ml/tensorflow/bencaine/babelfish/rs=6.3/ttl=90d/waymo_mod_head_04_29_21.v0/train/trainer_params.txt
\multicolumn{2}{l}{Optimizer} & \multicolumn{4}{l}{Adam \cite{kingma2014adam} ($\alpha = 1\mathrm{e}{-6}$, $\beta_1 = 0.9$, $\beta_2 = 0.999$)}  \\
\multicolumn{2}{l}{Batch size} & \multicolumn{4}{l}{\todo{64}} \\
\multicolumn{2}{l}{Weight initialization}  & \multicolumn{4}{l}{Xavier-Glorot \cite{glorot2010understanding}}  \\
\multicolumn{2}{l}{Weight decay}  & \multicolumn{4}{l}{None} \\

\bottomrule

\end{tabular}
\egroup
\vspace{0.2cm}
\caption{{\todo{OLD OLD} \bf \modelname\,architecture and training details.} The network receives as input a tensor of shape $[A, T, K]$ corresponding to $A$ agents, $T$ Time across $K$-dimensions. $K$ is the total number of input features (e.g. 3-D position, velocity, object type, bounding box size).  A subset of these inputs are masked. $G$ is the maximum number of road graph elements and $D$ is the total number of features. The output of the network is a tensor of shape $[F, A, T, 6]$ corresponding to predicting the 3-dimensional positions and associated uncertainties across $F$ futures. In our model $D=256$, $G=1400$, $T=91$, $A=128$, $K=7$ and $F=6$.}
% The top and bottom sections corresponds to the encoder and decoder, respectively.
\label{table:architecture-old}
\end{table*}


==> sections/old/architecture-table-old.tex <==
% /cns/oi-d/home/chauffeur/ml/tensorflow/bencaine/babelfish/rs=6.3/ttl=90d/waymo_mod_head_04_29_21.v0/train_train/model_analysis.txt
\begin{table*}[ht]
\scriptsize
\centering
\bgroup
\def\arraystretch{1.2}%  1 is the default, change whatever you need
\begin{tabular}{llcccccr}
\toprule
& Input & Operation & Queries & Keys/Values & Across & Atten Matrix & \# Param \\
\midrule
{\bf Embedder} \\
\todo{\it \tiny scene-encoder} & {\it Agents} & MLP + BN & -- & -- & -- & -- & 334080 \\
& {\it Dynamic RG} & MLP + BN & -- & -- & -- & -- & 337408 \\
& {\it Static RG} & MLP + BN & -- & -- & -- & -- & 270592 \\
%& {\it Static RG} & MLP + BN & -- & -- & -- & -- & 270080 \\

\midrule
{\bf Encoder} \\
%\midrule
\\
& $[A, T, D]$ & Transformer & Agents & Agents & Time & $[A, T, T]$ & 789824 \\
& $[A, T, D]$ & Transformer & Agents & Agents & Agents & $[T, A, A]$ & 789824 \\
\\
& $[A, T, D]$ & Transformer & Agents & Agents & Time & $[A, T, T]$ & 789824 \\
& $[A, T, D]$ & Transformer & Agents & Agents & Agents & $[T, A, A]$  &  789824 \\
\\
& $[A, T, D]$ & Transformer & Agents & Agents & Time & $[A, T, T]$ & 789824 \\
& $[A, T, D]$ & Transformer & Agents & Agents & Agents & $[T, A, A]$ & 789824 \\
\\
& $[A, T, D]$ & Transformer & Agents & Static RG & Time & $[T, A, G]$ & 789824 \\
& $[A, T, D]$ & Transformer & Agents & Dynamic RG & Time & $[T, A, G]$ & 789824 \\
\\
& $[A, T, D]$ & Transformer & Agents & Agents & Time & $[A, T, T]$ & 789824 \\
& $[A, T, D]$ & Transformer & Agents & Agents & Agents & $[T, A, A]$ & 789824 \\
\\
& $[A, T, D]$ & Transformer & Agents & Static RG & Time & $[T, A, G]$ & 789824 \\
& $[A, T, D]$ & Transformer & Agents & Dynamic RG & Time & $[T, A, G]$ & 789824 \\
\\
& $[A, T, D]$ & Transformer & Agents & Agents & Time & $[A, T, T]$ & 789824 \\
& $[A, T, D]$ & Transformer & Agents & Agents & Agents & $[T, A, A]$ & 789824 \\
\\

\midrule
{\bf Decoder} \\
& $[A, T, D]$ & Tile & -- & -- & -- & -- & 0 \\
& $[F, A, T, D]$ & Concat & -- & -- & -- & -- & 0 \\
\todo{\it \tiny split-into-futures} & $[F, A, T, D+F]$ & MLP & -- & -- & -- & -- & 68096 \\
\\
& $[F, A, T, D]$ & Transformer & Agents & Agents & Time & $[A, T, T]$ & 789824 \\
& $[F, A, T, D]$ & Transformer & Agents & Agents & Agents & $[T, A, A]$  &  789824 \\
\\
& $[F, A, T, D]$ & Transformer & Agents & Agents & Time &  $[A, T, T]$ & 789824 \\
& $[F, A, T, D]$ & Transformer & Agents & Agents & Agents & $[T, A, A]$  &  789824 \\
\\

& $[F, A, T, D]$ & Layer Norm & -- & -- & -- & -- & 512 \\

\todo{\it \tiny pose-predictor} & $[F, A, T, 7]$ & MLP & -- & -- & -- &  -- & 1799 \\

\todo{\it \tiny future-predictor}  & $[F, A, T, 6]$ & MLP + BN & -- & -- & -- &  -- & 395782 \\
\\
%\midrule
%{\bf Total} & & & & & & & 15,625,101 \\
\midrule
% https://source.corp.google.com/piper///depot/google3/waymo/shared/brain/behavior_understanding/params/waymo_mod.py;l=254
% /cns/oi-d/home/chauffeur/ml/tensorflow/bencaine/babelfish/rs=6.3/ttl=90d/waymo_mod_head_04_29_21.v0/train/trainer_params.txt
\multicolumn{2}{l}{Optimizer} & \multicolumn{4}{l}{Adam \cite{kingma2014adam} ($\alpha = 1\mathrm{e}{-6}$, $\beta_1 = 0.9$, $\beta_2 = 0.999$)}  \\
\multicolumn{2}{l}{Batch size} & \multicolumn{4}{l}{32} \\
\multicolumn{2}{l}{Weight initialization}  & \multicolumn{4}{l}{Xavier-Glorot \cite{glorot2010understanding}}  \\
\multicolumn{2}{l}{Weight decay}  & \multicolumn{4}{l}{None} \\

\bottomrule

\end{tabular}
\egroup
%\vspace{0.2cm}
\caption{{\bf \todo{OLD} \modelname\,architecture and training details.} The network receives as input a tensor of shape $[A, T, K]$ corresponding to $A$ agents, $T$ Time across $K$-dimensions. $K$ is the total number of input features (e.g. 3-D position, velocity, object type, bounding box size).  A subset of these inputs are masked. $G$ is the maximum number of road graph (RG) elements and $D$ is the total number of features. The output of the network is a tensor of shape $[F, A, T, 6]$ corresponding to predicting the 3-dimensional positions and associated uncertainties across $F$ futures. In our model $D=256$, $G=1400$, $T=91$, $A=128$, $K=7$ and $F=6$ for a total of 15,625,101 parameters.}
% The top and bottom sections corresponds to the encoder and decoder, respectively.
\label{table:architecture-old}
\end{table*}


==> sections/old/checklist.tex <==
\section*{Checklist}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Yes.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We include a Broader Impact statement describing the potential impact of this work.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We have ensured that our paper conforms with the ethical review guidelines.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We have included all relevant details to models introduced as well as the training details in main body of the paper and Appendix. Note that we do not intend to release the code for this model because our implementation is built upon proprietary internal formats and frameworks. Instead, we point readers to code accessing open-source datasets, and describe all of the details of the modeling approach in the main body of the paper and Appendix.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We have specified all training details in the main body of the paper and the Appendix.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Many of the experiments require a large amount of computation so we are not unable to report error bars. The variability during training provides a partial sense of the error bar and we observe very smooth training curves indicating that the validation dataset is quite large and the training is quite regular.}
    % Joint model.
    % https://tensorboard.corp.google.com/experiment/mldash:chauffeur:8119650759533646213/
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? \answerYes{We trained a model on a Cloud TPU v3-32 \cite{jouppi2017datacenter}. A single model took 3 days to converge over the course of 857K batches with batch size of 64 examples.}
    
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{Each asset has information pertaining to the license on their respective websites.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{As mentioned above, we do not intend to release the code for this model because our implementation is built upon proprietary internal formats and frameworks. Instead, we point readers to code accessing open-source datasets, and describe all of the details of the modeling approach in the main body of the paper and Appendix.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{We refer the reviewers and readers to the papers describing the original open-source datasets to see such details \cite{ettinger2021large,chang2019argoverse}.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{We are not aware of any personally identifiable information or offensive content in the two datasets discussed in the paper. That said, we refer the reviewers and readers to the papers describing the original open-source datasets for further details \cite{ettinger2021large,chang2019argoverse}.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> sections/old/intro-saved.tex <==
Motion planning in a real-world dynamic urban driving environment is a mission-critical problem for improving autonomous driving technology. 
The autonomous driving task is traditionally considered too difficult for a single system, let alone a learned system \cite{thrun2006stanley}. Thus, researchers have opted for a divide-and-conquer strategy by splitting the task into sequential subtasks \cite{zeng2019end}: (1) accurate perceiving the environment, (2) predicting the future motion of dynamic agents (behavior prediction), and (3) planning the future actions of the ego-agent. Such an approach produces interpretable representations where each component may exploit human-annotated datasets \cite{chang2019argoverse,ettinger2021large}, and can be examined to debug errors \cite{kim2018interpretability,kindermans2019reliability}. From a human organizational perspective, this structure offers the added benefit of allowing individual engineering teams to specialize on particular tasks.

Dividing the larger problem into subtasks achieves optimal performance when each subtask is truly independent. However such a strategy breaks down in important ways when this assumption does not hold. A system's predictions of what other agents will do next (the subtask of {\em behavior prediction}) directly influences what the ego-agent should decide to do next ({\em planning}). Similarly, just like all agent's behavior can influence all other agent's behavior, the ego-agent's actions will directly influence nearby agents. Despite a large body of recent work focusing on behavior prediction in isolation \cite{SocialGAN,alahi2016social,biktairov2020prank,buhet2020plop,casas2020spagnn,chai2019multipath,cui2019multimodal,gao2020vectornet,hong2019rules,lee2017desire,liang2020laneGCN,marchetti2020mantra,mercat2020multi,zhao2020tnt}, or sequentially with planning~\cite{bansal2019chauffeurnet,zeng2019end,sadat2020ppp}, we argue these problems should instead be solved jointly. Furthermore, we argue that when you look at behavior prediction through the lens of planning, it becomes advantageous to produce {\it joint} behavior predictions \cite{tang2019multiple,rhinehart2019precog,casas2020implicit, suo2021trafficsim,yeh2019diverse}, that is predictions that are internally consistent with each other, such that you can effectively plan against many diverse realistic future scenarios.


Our approach is instead directly inspired by recent developments in language models \cite{brown2020language,devlin2018bert}, where it was demonstrated that a single model trained on a large corpus may be re-used across an array of tasks by simply constructing an appropriate query. In the same manner, we seek a single architecture trained on a large dataset that may be queried to provide answers for the tasks of behavior prediction, conditional behavior prediction (i.e., answering counterfactuals by conditioning on different possible future observations of another agent), and goal-directed planning.

In this work, we present a single unified model that predicts a distribution over joint futures for all agents across time in a single inference pass.
Importantly, this approach can capture the large, cascading interactions between agents through conditioning, and allows the model to be trained simultaneously on the union of tasks, synergistically leveraging information from distinct kinds of supervision. 
% vrv: It's theoretically possible to make our model more agent-centric, with tradeoffs, so I think it's better to stay from language that implies that agent-centric is fundamentally flawed.
%This formulation eschews an agent-centric approach \cite{mercat2020multi,zhao2020tnt, wimp2020}, and instead develops a 
Our model uses a global representation for all agents in an environment---including the ego-agent / autonomous vehicle itself \cite{lee2017desire,hong2019rules,casas2020spagnn,salzmann2020trajectron++}. We employ a simple variant of self-attention \cite{vaswani2017attention} in which the attention mechanism is factorized across separate agent-time dimensions based on the nature of the problem. The resulting architecture requires nothing more than alternating attention between dimensions representing time and agents across the scene, resulting in a computationally efficient, uniform, and scalable architecture.

We find that the resulting model, termed a {\it \modelname}, achieves superior performance on standard per-agent independent behavior prediction benchmarks. Furthermore, we see strong indications that this learned model captures complex interactions between agents---including decisions by the autonomous vehicle---which are difficult to model with standard behavior prediction systems \cite{ettinger2021large,interactiondataset}. In subsequent sections we discuss which aspects of the system are critical for predictive performance and examine failure modes and opportunities for further refining the system. We hope that this work provides a compelling example for how
% pretraining on large corpora of driving behaviors, and
predicting joint, consistent futures of all agents in an environment opens new opportunities for critical tasks in autonomous vehicle technology.

In summary, our contributions in this work are:
\vspace{-6pt}

\begin{itemize}[leftmargin=0.5cm,rightmargin=0.5cm,itemsep=2pt,parsep=2pt]

\item A novel, scene-centric approach to representing joint future distributions over multiple agents in a single feed-forward network.

\item A Transformer-based architecture factored over agents, time, and road graph elements that exploits the inherent dependencies of the problem.  The resulting architecture is generic and integrates the world state in a unified way.

\item A unified multi-task training and inference framework in which a single model can accomplish the tasks of behavior prediction, conditional behavior prediction, and goal-directed planning.

\end{itemize}

% Although much work has vastly improved the perception capabilities of self-driving vehicles \cite{sun2020scalability,REF:lyftperception2019,geiger2013vision}, a critical challenge remains how to leverage all of this perceptual information to safely and efficiently arrive at the desired destination. 

%In the case of self-driving vehicles,
% navigtion is a separate roboics task, I think we should 
% directy call this planning.
% much work has focused on dividing the problem into {\it behavior prediction} (or motion forecasting) \cite{luo2018fast,casas2018intentnet}, i.e. predicting the potential future trajectories of agents such as vehicles and pedestrians, and {\it goal-directed planning} \cite{buehler2009darpa,montemerlo2008junior,ziegler2014trajectory}, i.e. selecting a route
% avenugopal: s/route/trajectory ? Since route is often used at a higher level (which roads)
% that efficiently arrives at the destination taking into account the actions of other agents. Such a division, however, suffers from several challenges.




%\begin{verbatim}
%---------------------
%    bensapp's take on key aspects of scene transformer:
%      * joint modeling: has been done before in 3-5 papers, but not in this way)
%      * Transformer layers: has been done before, but this axis-factored way is nicest I have seen)
%      * Training via masking: totally novel for this problem, lean into this?
%      * Unified BP/CBP/goal conditioning framework (= planner)
%      * global coordinates (has been done before with transformers, convnets, and GNNs)
%      * BP + planning models (has been done before)
%---------------------
%\end{verbatim}

%Overall Story
%\begin{enumerate}
%    \item BP models traditionally
%    \begin{enumerate}
%        \item \st{Modeled each agent separately, and used an agent-centric representation}
%        \item Had many choices of architectures for the network
%    \end{enumerate}
%    \item \st{Few models perform joint modeling to capture agent-agent interactions}
%    \item We find that
%    \begin{enumerate}
%        \item \st{Transformers work well here, no need for different archs. Simplicity in modeling.}
%        \item Global coordinates through positional embeddings work well too.
%        \item Allows us to regress exact xyz
%    \end{enumerate}
%    \item \st{Together, these provide a simple and effective framework for joint modeling.}
%\end{enumerate}

%Key Contributions
%\begin{enumerate}
%    \item \st{Architecture: Modeling with transformers}
%    \item Global Coordinates: Using positional embeddings work
%    \item \st{Joint scene modeling}
%    \item \st{Different masking strategies can reflect different tasks (BP, CBP, etc)}
%\end{enumerate}





==> sections/old/results-old.tex <==
\section{Results}

\input{sections/motivation-figure}

We train the \modelname on behavior prediction tasks from the Waymo Open Motion Dataset (\wmod) \cite{ettinger2021large} and the Argoverse dataset \cite{chang2019argoverse}. The \wmod dataset consists of 104,000 run segments (each 20 seconds in duration) over 1,750 km of unique roadways containing 7.64 million unique agent tracks. The Argoverse dataset consists of 324,000 run segments (each 5 seconds in duration) over 290 km of unique roadways containing 11.7 million unique agent tracks. Each model is trained on a Cloud TPU \cite{jouppi2017datacenter} (See Appendix for all training details). We demonstrate that the resulting model achieves best published performance across these datasets.

For the Argoverse dataset, we train and evaluate the model solely on the behavior prediction task. Thus, we only employ the behavior prediction mask (Figure \ref{fig:model-architecture-diagram}, left) for training the model. For the \wmod we train the model with all masks jointly, selecting a mask strategy for each batch uniformly at random. We evaluate the \wmod on behavior prediction, conditional behavior prediction and goal-directed planning. For all models, we evaluate the quality of $k$ weighted trajectory hypotheses using a suite of standard evaluation metrics (See Methods).

% {"brier-minFDE (K=6)": 1.9382042855377244, "minFDE (K=6)": 1.2871143138000782, "MR (K=6)": 0.1352520379304608, "minADE (K=6)": 0.8407221633190511, "DAC (K=6)": 0.9898071484330025, "minFDE (K=1)": 4.006746863124136, "MR (K=1)": 0.5953060414880411, "minADE (K=1)": 1.8069812509575218, "DAC (K=1)": 0.9916819164864416, "minADE (K=3)": 1.174250466410473, "minFDE (K=3)": 2.3263747074043177, "DAC (K=3)": 0.9885551702221121, "MR (K=3)": 0.3186209897239676, "p-minADE (K=6)": 2.555927143255828, "p-minFDE (K=6)": 3.0023192937368597}

\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{c|ccc}
    \toprule
    Method & minADE$\,\downarrow$ & minFDE$\,\downarrow$ & MR$\,\downarrow$ \\
    \midrule
     Jean \citep{mercat2020multi} & 0.97 & 1.42 & 0.13 \\
     WIMP \citep{wimp2020} & 0.90 & 1.42 & 0.17 \\
     TNT \citep{zhao2020tnt} & 0.94 & 1.54 & 0.13 \\
     LaneGCN \citep{liang2020laneGCN} & 0.87 & 1.36 & 0.16 \\
     TPCN \citep{ye2021tpcn} & 0.85 & 1.35 & 0.16 \\
     mmTransformer \citep{liu2021multimodal} & 0.84 & 1.34 & 0.15 \\
     HOME \citep{HOME2021} & 0.94 & 1.45 & {\bf 0.10} \\
     %MulitPath++ & 0.89 & 1.50 & 0.131 \\
     \modelname (Ours) & {\bf 0.80} & {\bf 1.23} & 0.13 \\
     \bottomrule
\end{tabular}
\vspace{0.2cm}
\caption{\textbf{Predictive performance on Argoverse behavior prediction.} Results reported on {\it test} split for vehicles \cite{chang2019argoverse}. Reported are the minADE, minFDE for $k=6$ predictions \cite{alahi2016social,pellegrini2009you}, and the Miss Rate (MR) \cite{chang2019argoverse} within 2 meters of the target. All results are reported for $t=3$ seconds. Since the task specifies only one agent to predict per scene, marginal and joint are equivalent with our method. \label{table:argoverse-test-results}}
\vspace{-0.2cm}
\end{table}

% Some baseline numbers gathered from here:
% https://docs.google.com/document/d/1pKeoR0zzl21BoLjQ8fSe_nUt5hVSNueBTw1Yes5yPcA/edit
\begin{table}[t]
\centering
\footnotesize
\bgroup
\def\arraystretch{1.05}%  1 is the default.
\resizebox{\linewidth}{!}{
\begin{tabular}{cc|ccc|ccc|ccc|ccc}
    \toprule
    \multicolumn{2}{c|}{\multirow{2}{*}{{\bf Motion Prediction}}} & \multicolumn{3}{c|}{minADE$\,\downarrow$} & \multicolumn{3}{c|}{minFDE$\,\downarrow$} & \multicolumn{3}{c|}{MR$\,\downarrow$} & \multicolumn{3}{c}{mAP$\,\uparrow$} \\
    & & veh & ped & cyc & veh & ped & cyc & veh & ped & cyc & veh & ped & cyc\\ 
    \midrule
    {\it valid} & & & & & & & & & & & \\
     & LSTM baseline \cite{ettinger2021large} & 1.34 & 0.63 & 1.26 & 2.85 & 1.35 & 2.68 & 0.25 & 0.13 & 0.29 & 0.23 & 0.23 & \textbf{0.20} \\
     % From leaderboard submission
     & ours (marginal) & {\bf 1.17} & \textbf{0.59} & \textbf{1.15} & \textbf{2.51} & \textbf{1.26} & \textbf{2.44} & \textbf{0.20} & \textbf{0.12} & \textbf{0.24} & \textbf{0.26} & \textbf{0.27} & \textbf{0.20} \\
     % From leaderboard submission
     & ours (joint, bp-only) & 1.53 & 0.90 & 1.63 & 3.48 & 2.09 & 3.77 & 0.28 & 0.30 & 0.37 & 0.20 & 0.16 & 0.13\\
     % At 371.2K steps
     % https://tensorboard.corp.google.com/experiment/mldash:chauffeur:5237978701955273581/#scalars&regexInput=Dev&tagFilter=joint_metrics%2FVehicle_at_8s&_smoothingWeight=0
     & ours (joint, multi-task) & 1.56 & 0.89 & 1.60 & 3.56 & 2.06 & 3.68 & 0.29 & 0.29 & 0.37 & 0.19 & 0.15 & 0.15\\
     \midrule
    {\it test} & & & & & & & & & & & & \\
     & LSTM baseline \cite{ettinger2021large} & 1.34 & 0.64 & 1.29 & 2.83 & 1.35 & 2.68 & 0.24 & 0.13 & 0.29 & 0.24 & 0.22 & 0.19\\
     & ours (marginal) & \textbf{1.17} & \textbf{0.60} & \textbf{1.17} & \textbf{2.48} & \textbf{1.25} & \textbf{2.43} & \textbf{0.19} & \textbf{0.12} & \textbf{0.22} & \textbf{0.27} & \textbf{0.23} & \textbf{0.20}\\
     & ours (joint, bp-only) & 1.52 & 0.91 & 1.61 & 3.43 & 2.09 & 3.68 & 0.28 & 0.30 & 0.37 & 0.19 & 0.16 & 0.19\\
     & ours (joint, multi-task) & 1.55 & 0.91 & 1.64 & 3.50 & 2.08 & 3.75 & 0.28 & 0.29 & 0.38 & 0.19 & 0.16 & 0.19\\
     \bottomrule
\end{tabular}}
\egroup
\\ \vspace{0.2cm}
\bgroup
\def\arraystretch{1.05}%  1 is the default.
\resizebox{\linewidth}{!}{
\begin{tabular}{cc|ccc|ccc|ccc|ccc}
    \toprule
    \multicolumn{2}{c|}{\multirow{2}{*}{{\bf Interaction Prediction}}} & \multicolumn{3}{c|}{minSADE$\,\downarrow$} & \multicolumn{3}{c|}{minSFDE$\,\downarrow$} & \multicolumn{3}{c|}{SMR$\,\downarrow$} & \multicolumn{3}{c}{mAP$\,\uparrow$}\\
    & & veh & ped & cyc & veh & ped & cyc & veh & ped & cyc & veh & ped & cyc\\ 
    \midrule
    {\it valid} & & & & & & & & & & &\\
     & LSTM baseline \cite{ettinger2021large} & 2.42 & 2.73 & 3.16 & 6.07 & 4.20 & 6.46 & 0.66 & 1.00 & 0.83 & 0.07 & \textbf{0.06} & 0.02 \\
     % From leaderboard submission
     & ours (marginal) & 2.04 & 1.62 & 2.28 & 4.94 & 3.81 & 5.67 & 0.54 & 0.63 & 0.72 & \textbf{0.11} & 0.05 & 0.03 \\
     % From leaderboard submission
     & ours (joint, bp-only) & \textbf{1.72} & \textbf{1.38} & 1.96 & \textbf{3.98} & \textbf{3.11} & 4.75 & \textbf{0.49} & \textbf{0.60} & 0.73 & \textbf{0.11} & 0.05 & 0.03  \\
     % At 371.2K steps
     % https://tensorboard.corp.google.com/experiment/mldash:chauffeur:5237978701955273581/#scalars&regexInput=Dev&tagFilter=joint_metrics%2FVehicle_at_8s&_smoothingWeight=0
     & ours (joint, multi-task) & \textbf{1.72} & 1.39 & \textbf{1.94} & 3.99 & 3.15 & \textbf{4.69} & \textbf{0.49} & 0.62 & \textbf{0.71} & \textbf{0.11} & \textbf{0.06} & \textbf{0.04} \\     
     \midrule
    {\it test} & & & & & & & & & & & \\
     & LSTM baseline \cite{ettinger2021large} & 2.46 & 2.47 & 2.96 & 6.22 & 4.30 & 6.26 & 0.67 & 0.89 & 0.89 & 0.06 & 0.03 & 0.03\\
     % At 857.6K steps
     & ours (marginal) & 2.08 & 1.62 & 2.24 & 5.04 & 3.87 & 5.41 & 0.55 & 0.64 & 0.73 & 0.08 & \textbf{0.05} & 0.03 \\
     & ours (joint, bp-only) & 1.76 & \textbf{1.38} & \textbf{1.95} & 4.08 & \textbf{3.19} & \textbf{4.65} & \textbf{0.50} & \textbf{0.62} & \textbf{0.70} & 0.10 & \textbf{0.05} & \textbf{0.04}\\
     & ours (joint, multi-task) & \textbf{1.74} & 1.41 & \textbf{1.95} & \textbf{4.06} & 3.26 & 4.68 & \textbf{0.50} & 0.64 & 0.71 & \textbf{0.13} & 0.04 & 0.03\\
     \bottomrule
\end{tabular}}
\egroup
\vspace{0.2cm}
\label{table:wmod-results-old}
\caption{\textbf{Predictive performance on Waymo Open Motion Dataset behavior prediction} \cite{ettinger2021large}. Top: Marginal predictive performance based on the {\it standard} splits of the validation and test datasets. Bottom: Joint predictive performance based on the {\it interactive} splits of the validation and test datasets. Reported are the min(S)ADE, min(S)FDE for $k=6$ predictions \cite{alahi2016social,pellegrini2009you}, and the Miss Rate (MR) \cite{chang2019argoverse} within 2 meters of the target. Results for the {\it Motion Prediction} section use traditional marginal metrics, while results for the {\it Interaction Prediction} use joint, scene-level variants of these metrics (see \cite{ettinger2021large}). All results are reported at $t=8$ seconds. See Appendix for $t=3$ and $t=5$ seconds.}
\vspace{-0.6cm}
\end{table}

\subsection{Behavior prediction}

{\bf Argoverse.} 
% We start by validating a simplified version of \modelname for the behavior prediction task on the Argoverse dataset. We specify the task of behavior prediction by masking out the future positions of agents in the scene. 
The Argoverse task requires that we predict a single agent. We use a masking strategy that provides the model with all the agents as input, but with their futures masked out. During training, the model is only required to predict the future of the single agent of interest.  Our best Argoverse model uses $D=512$ feature dimensions and label smoothing for trajectory classification.  Our model achieves state-of-the-art results compared to published\footnote{We chose to exclude comparing to public leaderboard entries that have not been published since their details are not available, but note that our results are competitive on the leaderboard as of the submission date.} prior work in terms of minADE/minFDE (Table \ref{table:argoverse-test-results}).
% We also find that the model achieves \todo{state of the art results} on the validation split of Argoverse (Table \ref{table:argoverse-validation-results} in Appendix). 
% These scores indicate that the model predicts the single agent accurately even in this simplified setting in which the model is not conditioned on other agent's behaviors.

{\bf Waymo Open Motion Dataset (\wmod).} Next we evaluate the performance of our model with $D=256$ on the recently released Waymo Open Motion Dataset \cite{ettinger2021large}. \wmod provides two separate evaluation tasks with unique metrics and associated validation and test data sets. The first task is the {\it Motion Prediction} challenge, which is a standard motion forecasting task where up to 8 of the scene's agents are chosen to have their top 6 trajectory predictions evaluated independently. The second is the {\it Interaction Prediction} challenge, which tasks the model with predicting the trajectories of two interacting agents {\it jointly}. The metrics for the {\it Interaction Prediction} task are {\it joint} variations of the common minADE, minFDE, and Miss Rate metrics, and measure the quality of the joint prediction of both agents within up to 6 predicted futures.

To fully compare the marginal and joint formulations of our model, we evaluate the product of these models and datasets. That is, we evaluate the marginal model on the {\it Motion Prediction} challenge, and then evaluate it on the {\it Interaction Prediction} challenge by converting our marginal predictions to joint ones mirroring the methodology in \cite{ettinger2021large}\footnote{We take the top 6 pairs of trajectories from the combination of both agent's trajectories for 36 total pairs.}. We then evaluate our joint model on the {\it Motion Prediction} challenge to see how it would fare as a marginal model, despite being trained to solve the harder joint problem, and then we evaluate it as a true joint model using joint metrics on the {\it Interaction Prediction} challenge. 

We find that the marginal model achieves state-of-the-art performance over the provided baseline (Table \ref{table:wmod-results-old}, top) on the {\it Motion Prediction} challenge, demonstrating the strength of our general architecture. We next show that the same architecture, instead trained with the joint loss formulation, performs worse on marginal metrics on the same {\it Motion Prediction} challenge.  The story flips when we look at the {\it Interaction Prediction} challenge (Table \ref{table:wmod-results-old}, bottom), which evaluates the model's joint predictions with joint scene-level metrics. Our joint model easily outperforms both the baseline \cite{ettinger2021large} and our own marginal model's predictions converted to joint predictions on metrics such as minSADE \cite{casas2020implicit}. This shows that beyond the strength of our overall architecture and approach, that explicitly training a model as a joint model significantly improves joint performance on joint metrics, at the cost of that models performance on marginal metrics. A notable observation is that even though the {\it Interaction Prediction} task only requires predicting the joint trajectories of two agents, our method is fully general and predicts joint consistent futures of all agents.

%We show that our architecture, when trained and evaluated as a marginal model, achieves state of the art results on all metrics on the \wmod, demonstrating the strength of the architecture and the lack of limitations of a scene-centric representation. Then, 
%{\bf Waymo Open Motion Dataset (\wmod).} We next evaluate the predictive performance of the marginal model on the recently released Waymo Open Motion Dataset \cite{ettinger2021large}. \wmod provides two separate evaluation datasets: the {\it standard} split that measures cross-validated generalization error, and the {\it interactive} split that measures cross-validated generalization on scenarios that focus on challenging interactive behaviors between agents \footnote{The standard and interactive splits are also termed {\it motion prediction} and {\it interaction prediction}, respectively, on the public leaderboard at \url{https://waymo.com/open/challenges/}.}. 
% Table \ref{table:wmod-results-old} (top) reports the same performance metrics for the marginal version of the model on the validation and test splits on the standard split of the data. 
%We find that the marginal model achieves state-of-the-art performance over the provided baseline (Table \ref{table:wmod-results-old}, top). Notably, the marginal model performs worse on the interactive split (Table \ref{table:wmod-results-old}, bottom) reflecting the inability of the model to take into account the interactions between agents \footnote{For additional results for behavior prediction on the \wmod at $t=5$ and $t=3$ seconds, please see Table \ref{table:wmod-results-t5} and \ref{table:wmod-results-t3} in the Appendix, respectively.}.

%The worse performance of the marginal model on the interactive version of \wmod suggests that modeling the joint, consistent behavior of all agents may be able to repair the performance. We test this hypothesis by training a model to predict the futures of all agents jointly, and test the performance on both the standard and interactive datasets. First, we find that joint future model performs slightly worse on marginal metrics when evaluated on the motion prediction task in the standard split. However, we find that the model performs notably better on joint metrics and achieves state-of-the-art results on the challenging interactive split of the data (Table \ref{table:wmod-results}, bottom).

{\bf Multi-task prediction.} The larger goal of this work is to develop a method amenable to solving multiple prediction tasks, including behavior prediction, conditional behavior prediction and goal-directed planning.  We next ask if \modelname can be trained as a multi-task model using the same architecture, but with a mix of masking strategies that correspond to each task. During training, we supply masks corresponding to the three tasks with a probability $1/3$ each.

% We discuss the evaluation of the multi-task model for behavior prediction, and reserve the analysis of conditional behavior prediction and goal-directed planning for subsequent sections.   <-- redundant with the end of the next paragraph.

% Table \ref{table:wmod-results} shows the resulting performance for the multi-task model on the standard and interactive splits for the \wmod. 
We find that the multi-task model trained with a joint loss achieves behavior prediction metrics comparable to the joint prediction model (Table \ref{table:wmod-results}) trained on BP only, despite being trained with additional masks for conditional behavior prediction and goal-directed planning. This indicates that a jointly-trained multi-task model is a viable strategy for solving many behavior prediction problems.
%, but reserve the analysis for conditional behavior prediction and goal-directed planning for subsequent sections.

\subsection{Understanding the trade-offs between the joint and marginal models}


\begin{figure*}[t]
\centering
\includegraphics[width=0.3\textwidth]{figures/joint_marginal_minade.png} %/Overlap-Scatter.jpg} 
\hspace{0.1cm}
%\includegraphics[width=0.24\textwidth]{figures/joint_marginal_overlap.png} %Overlap-Difference.pdf}
%\includegraphics[width=0.24\textwidth]{figures/slicing/original_minADE_average_sdc_speed_slicing_cut.png}
\includegraphics[width=0.3\textwidth]{figures/slicing/original_minADE_num_ade_valid_slicing_main.png}
\hspace{0.1cm}
\includegraphics[width=0.3\textwidth]{figures/slicing/joint_marginal_overlap_num_pred_agents.png}
%\includegraphics[width=0.24\textwidth]{figures/slicing/original_overlaps_average_sdc_speed_slicing_cut.png}
\caption{\textbf{Quantitative comparison of the marginal and joint prediction models.} Left: Cumulative distribution of the minADE for the marginal and joint models evaluated on the motion prediction task. The mean minADE for the marginal model is lower than the joint model (marginal $=1.05m$ vs joint $=1.35m$). Center: The minADE broken down as a function of number of predicted agents. When there are more agents, producing internally consistent predictions is more challenging, and hence the joint model performs slightly worse. Right: Overlap rate between pairs of agent predictions. The joint model produces internally consistent predictions with lower inter-prediction overlap rates. \label{figure:joint-marginal-comparison}}
%Comparison of the overlap metric between the marginal and joint prediction model. 
%Plot shows the number of predicted trajectories with a non-zero overlap with the bounding box of any other agent within the scenario as a fraction of the number of predicted agents within the scenario. Each dot represents the number of overlaps that occur on a single scenario for the joint and marginal models, respectively. The line denotes line of equality while the green + marks the mean overlap fraction for joint and marginal models at \todo{0.010462 and 0.021274} respectively. Right:  \label{figure:joint-marginal-comparison}}
\end{figure*}


While the joint BP-only model performs better on the interactive prediction task than the marginal model, it performs worse on the motion prediction task. This is because the joint model is trained to produce predictions that are internally consistent between agents, while the marginal model does not. In this section, we examine this quality difference and the internal consistency of the predictions from both models.


In the \wmod dataset, each example has a different number of agents to be predicted. By slicing the {\it marginal} minADE results based on the number of agents to be predicted (Figure \ref{figure:joint-marginal-comparison}, center), we find that the joint model performs worse as there are more predicted agents, while the marginal model performs the same. This is expected: when there are more agents, the joint model has a more difficult task since it needs to produce internally consistent predictions. We note that this result is encouraging as it shows that the joint model may not need to predict an exponential number of trajectories to perform competitively with the marginal model.\footnote{One might expect a joint model to need an exponential number of trajectories to match the combinatorial possibilities of a marginal model. However, when many agents are interacting, the number of realistic scenarios can be more constrained by the interactions.} 

However, when more agents are to be predicted, the possibility of interactions are higher and we would expect that the joint model is able to capture these interactions through internally consistent predictions. We measure the models' internal consistency by selecting the best trajectory and measuring the {\it inter-prediction overlap rate} (details in Appendix). We find that the joint model has a consistently lower inter-prediction overlap rate, showing that it is able to capture the interactions between agents. The ability to model interactions enables the model to be suitable for CBP and GDP tasks, which we discuss in following sections.


% In this section, we next examine the benefits of the joint future prediction by analyzing the differences in the predictive performance between the marginal and joint \modelname models. Table \ref{table:wmod-results} already suggests that a joint model may selectively perform better or worse than a marginal model depending on the selection of data and the manner of evaluation. We next examine this closer by examining the relative performance of the marginal and joint models across individual scenes.

% Figure \ref{figure:joint-marginal-comparison} (left-most) shows the cumulative distribution of the minADE for the marginal and joint models evaluated with marginal metrics. As seen previously, the marginal model again exhibits a lower minADE (marginal $=1.05\,m$ vs joint $=1.35\,m$). We see that both models however demonstrate systematic variability across multiple dimensions. For instance, minADE is systematically increases as the average AV speed increases in the marginal model (Figure \ref{figure:joint-marginal-comparison}, right panel); likewise, the minADE systematically grows as the number of agents that must be predicted increases, or the number of moving agents in the scene increases (Appendix, Section \ref{section:slicing-results}). 


% Given that the joint model's minADE is higher than the marginal model's, one might ask why the joint model performs better with the {\it Interaction Prediction} task (Table \ref{table:wmod-results}, bottom). We can gain some insight into this discrepancy by examining the rate of overlaps between pairs of agents in the trajectory predictions (Figure \ref{figure:joint-marginal-comparison}). The overlap rate measures the frequency at which two agents overlap in space and time above some threshold (see Appendix for details) and stands as a proxy for evaluating the consistency of a joint future prediction. Notably, we find that the rate of overlap between agents is significantly lower in the joint model than the marginal model (Figure \ref{figure:joint-marginal-comparison}). The mean overlap rate drops from \todo{$XXX$} to \todo{$XXX$} from the marginal to the joint model. 


% [\todo{to reword based on new fig: Finally, we see that this systematic decrease in the overlap persists across various slices of data such as the average speed of the AV (Figure \ref{figure:joint-marginal-comparison}). These results indicate that although the joint model may less accurately predict individual trajectories, the overall metrics are improved because the joint model better captures the interactions between agents in the environment.}]

\subsection{Conditional behavior prediction with a multi-task model}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.325\textwidth]{figures/cbp_red.png}
% %\includegraphics[width=0.325\textwidth]{figures/cbp_blue.png}
% \includegraphics[width=0.325\textwidth]{figures/cbp_ratio.png}
% \caption{\textbf{Multi-task model is able to leverage additional information in CBP mode.} Left: Cumulative probability of the minADE in CBP (red) and BP (black) masking strategies. CBP achieves a mean minADE of 1.25 for CBP, while BP obtains 1.34. Right: Average ratio of minADE (BP/CBP) as a function of average speed of agents in the scene. CBP outperforms when the ratio is greater than 1.0, and shows more improvement at higher speeds. \label{fig:cbp-quantitative}}
% \end{figure*}

Given that the joint prediction model better captures interactions, we next investigate the additional benefits in training a multi-task model trained on BP, CBP, and GDP. We train a single multi-task model, where each task is presented during training $1/3$ of the time, and run it at inference with different masks to evaluate its ability to perform different tasks.

The CBP task provides the model with the full trajectory of a single specified agent, and requires the model to produce future trajectories for the other agents.
% We first examine how a multi-task model is able to exploit additional information at inference time on a conditional behaviour prediction (CBP) task.
% Specifically, we compare the same multi-task model run at inference with a CBP or BP mask and ask if the resulting CBP model provides superior predictive performance.
% by comparing against the 
%In this section we detail the conditional behavior prediction (CBP) aspect of the multi-task model. As illustrated in Figure~\ref{fig:model-architecture-diagram}, CBP corresponds to the masking strategy where the future of one agent's trajectory is shown. 
We focus on the interactive split of \wmod in order to provide a meaningful test bed for CBP.
%We focus on the interactive split of \wmod, where each scene contains two agents that are ``interacting'', making them a useful test bed for CBP.
To fairly compare to BP, for each scene we average the two agents' minADE when conditioned on the ground truth of the other.
We compare the same multi-task model's performance in both BP and CBP inference modes.  The CBP minADE is 0.09 lower than the BP counterpart (1.25 vs 1.34), demonstrating that \modelname is able to utilize useful information from the future (when available) to improve behavior prediction. 
% Figure~\ref{fig:cbp-quantitative} (left) shows the cumulative distribution of minADE over the interactive validation set, where the CBP minADE is the numerical average of the two agents' minADE when conditioned on the other. 
% Overall, the conditional behavior prediction minADE is 0.09 higher than the behavior prediction counterpart, demonstrating that \modelname is able to utilize useful information from the future (when available) to improve behavior prediction.
% The advantage of CBP over BP becomes greater if the scene in general has higher speed (Figure~\ref{fig:cbp-quantitative}, right).  

%\begin{enumerate}
%    \item Visualizations of scenarios where it helps?
%    \item \st{Quantitative measurements of minADE/other thing improvements? Interactive on 2 agent measurements. BP vs CBP where they leak information.}
%\end{enumerate}

\subsection{Goal-directed planning with a multi-task model}

\begin{figure*}[t]
\centering
\begin{tabular}{p{0.3\textwidth}p{0.3\textwidth}p{0.3\textwidth}}
%\textit{Scenario A} & \textit{Scenario B} & \textit{Scenario C} & \textit{Scenario D} \\
\textit{Scenario A} & \textit{Scenario B} & \textit{Scenario C}\\
\end{tabular}

%\includegraphics[width=\textwidth]{figures/planning/PlanningAll.png}
\includegraphics[width=\textwidth]{figures/planning/PlanningAllDropA.png}


%\includegraphics[width=0.22\textwidth]{figures/planning/1-Left-Turn.png}
%\includegraphics[width=0.22\textwidth]{figures/planning/2-Left-Turn.png}
%\includegraphics[width=0.22\textwidth]{figures/planning/3-Lane-Change.png}
%\includegraphics[width=0.22\textwidth]{figures/planning/4-Nudging.png} \\

%\includegraphics[width=0.22\textwidth]{figures/planning/1-Yielding.png}
%\includegraphics[width=0.22\textwidth]{figures/planning/2-U-Turn.png}
%\includegraphics[width=0.22\textwidth]{figures/planning/3-No-Lane-Change.png}
%\includegraphics[width=0.22\textwidth]{figures/planning/4-Stopping.png}
% \caption{\textbf{Goal-directed planning navigates to directed location.} Rectangles indicate vehicles on the road. Lines indicate the road graph (RG) colored by the type of lane marker. \todo{Describe the color legend for the lanes.} Circles indicate predicted trajectory for each agent. Star indicates selected goal for AV. Each column represents a scenario in which the AV is directed to perform one of two actions taking into account the dynamics of other agents. (A) AV instructed to either turn left or yield to oncoming traffic at intersection. (B) AV instructed to either make left turn or U-turn at intersection. (C) AV instructed to either change lanes or remain in the same lane. (D) AV instructed to stop to allow oncoming vehicle to correctly turn left, or adjust to the side in a narrow passage so that the oncoming vehicle has enough space to pass. \label{fig:planning-visualizations}}
%\caption{\textbf{Goal-directed planning navigates AV to selected goal positions.} Rectangles indicate vehicles on the road. Lines indicate the road graph (RG) colored by the type of lane marker. Circles indicate predicted trajectory for each agent. Star indicates selected goal for AV. Each column represents a scenario in which the AV is directed to perform one of two actions taking into account the dynamics of other agents. (A) AV instructed to either turn left or prepare for U-turn at intersection. (B) AV instructed to either change lanes or remain in the same lane. (C) AV instructed to stop to allow oncoming vehicle to turn left, or adjust to the side in a narrow passage so that the oncoming vehicle has enough space to pass. (D) AV instructed to either proceed straight or turn right at the intersection. \label{fig:planning-visualizations}}
\caption{\textbf{Goal-directed planning navigates AV to selected goal positions.} Rectangles indicate vehicles on the road. Lines indicate the road graph (RG) colored by the type of lane marker. Circles indicate predicted trajectory for each agent. Star indicates selected goal for AV. Each column represents a scenario in which the AV is directed to perform one of two actions taking into account the dynamics of other agents. (A) AV instructed to either change lanes or remain in the same lane. (B) AV instructed to stop to allow oncoming vehicle to turn left, or adjust to the side in a narrow passage so that the oncoming vehicle has enough space to pass. (C) AV instructed to either proceed straight or turn right at the intersection. \label{fig:planning-visualizations}}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=0.325\textwidth]{figures/planning/planningMinAde.png}
\includegraphics[width=0.325\textwidth]{figures/planning/planningSlicing.png}
\caption{\textbf{Analysis of the multi-task model for goal-directed planning.} Left: Cumulative probability of the AV minADE in planning (blue) and BP (black) masking strategies. 
Right: AV minADE for planning (blue) and BP (black) as a function of AV speed (averaged over the ground truth trajectory).
\label{fig:planning-quantitative}}
\end{figure*}

% We demonstrated in the previous section that the unified multi-task model presented in the previous section trained with all masking strategies works well on behavior prediction and conditional behavior prediction. 
We next examine how the \textit{same} multi-task model in the previous section performs on goal-directed planning (GDP). 
% We define goal-directed planning as predicting the AV's trajectory given a position goal as well as the history of the AV and other agents.  % this sentence is the same as the ntx
% Original, though the first 2 sentences were modifed and cannot be undone due to the overleaf multil-user undo issue. 
% We supply the model with a masking strategy where the final position of the AV is provided along with the positions of all agents up to the current time (Figure \ref{fig:model-architecture-diagram}). We ask the model to fill in the AV trajectory. This final task is less well defined in the literature, but as a proof of principle we showcase several visualizations of the previously trained model in a goal-directed scenario. We show side-by-side comparisons of the same multi-task model in which we show the highest likelihood trajectory for all agents conditioned two different endpoints selected by ourselves at inference time. For each of the artificially selected endpoints, we observe that the model  produces a plausible trajectory to arrive at the endpoints based on the expected interactions with other agents.
% run inference on the interactive split of the \wmod on two models: (1) the jointly trained behavior prediction model and (2) the multi-task trained model. We calculate the \todo{difference} in the minADE for the final prediction of the \todo{AV} between the two models. Figure \ref{fig:planning-quantitative} shows the cumulative distribution of the difference in the minADE between these two models. Note that more \todo{finish me}.
Specifically, we want to aid a full planning system that evaluates potential AV goal destinations by providing consistent, joint futures of all agents.  We supply the model at inference time with a GDP mask where the final position of the AV is specified along with the state history of AV and all agents (Figure \ref{fig:model-architecture-diagram}), and ask the model to fill in the AV trajectory. 
This task is less well-defined in the literature, but as a proof of principle we showcase several visualizations of the multi-task model in goal-directed scenarios.
% Specifically, Figure \ref{fig:planning-visualizations} top and bottom rows show the AV navigating to two artificially selected goal positions we selected at inference time. 
Qualitatively, we demonstrate that our model produces reasonable trajectories to arrive at the goal positions, even when they differ from the ground truth, across a diverse repertoire of behaviors (Figure \ref{fig:planning-visualizations}). 
Critically, we observe that AV goal conditioning impacts the predicted behavior of \emph{other agents} in a consistent, realistic manner.

Quantitatively, we verify that our model can effectively use the privileged information of the final ground truth endpoint
%We quantify the effectiveness of the multi-task model for GDP
by re-purposing the behavior prediction metrics for measuring the performance of the AV prediction. We compare the performance of the multi-task model under two different masking strategies {\it at inference time}: (1) A masking strategy for behavior prediction and (2) A masking strategy for goal-directed planning. 
We find that the minADE for the AV is decreased for the interactive split of the \wmod (Figure \ref{fig:planning-quantitative}) when the privileged information is made available to the multi-task model.
%We finally ask how the multi-task model is able to predict the trajectory of the AV under each strategy -- if the multi-task model is able to exploit the additional oracle information, the minADE for the trajectory should be superior for the goal-directed masking strategy. We find that the minADE for the AV is significantly decreased for the interactive split of the \wmod (Figure \ref{fig:planning-quantitative}). On average the minADE is $1.6\times$ higher for the behavior prediction mask than the goal-directed planning mask, indicating that the model is able to exploit the additional information about other agents and the goal at inference time. 
When we break down the minADE across AV speeds, we find that the gains of employing a goal-directed planning mask are most pronounced at lower speeds, peaking at roughly  $2\times$ reduction in minADE.
This latter property is particularly advantageous as many complex interactive maneuvers
%(e.g. nudging)
occur in crowded environments at low speeds.

%Namely, we supply the model with an AV goal position identical to the ground truth position at the last time step in the \wmod interactive split. 
%Figure \ref{fig:planning-quantitative} shows the AV minADE compared to the same multi-task model inferenced with the unconditioned BP masking strategy. The left shows the cumulative probability while the right shows the ratio of BP and planning minADE as a function of AV speed.
%It is clear that the multi-task model can effectively utilize the supplied AV goal position to produce higher quality AV planning solutions (BP minADE is 1.61x larger).
%The minADE advantage of goal-directed planning is particularly noticeable at low AV speeds.
%This is a desirable property as many of the most complex maneuvers such as nudging in crowded environments occur at low speeds.
% This is likely due to the fact that minADE is larger masking strategies as for both metric is sensitive to minor errors in predicted speed at high speeds




==> sections/old/results-very-old.tex <==
\section{OLD Results (For reference)}

% \begin{table}[t]
% \centering
% \footnotesize
% \bgroup
% \def\arraystretch{1.1}%  1 is the default.
% %\parbox{.44\linewidth}{
% \begin{tabular}{c|cccc}
%     \toprule
%     %Waymo Open Motion &  minADE ($k$=$6$) & minFDE ($k$=$6$) & MissRate\,$@\,2m$ \\
%     WOMD & minADE$\,\downarrow$ & minFDE$\,\downarrow$ & MR$\,\downarrow$ & mAP$\,\uparrow$\\
%     \midrule
%      SEERNet & 1.34 & - & 0.25 & \todo{?}\\
%      ours (marginal) & 1.24 & 2.85 & 0.46 & \todo{?} \\
%      ours (joint) & 1.54 & 3.75 & 0.49 & \todo{?} \\ 
%      \bottomrule
% \end{tabular}
% %}
% \\ \vspace{0.1cm}
% %\egroup
% %\vspace{0.3cm}
% %\hfill
% %\bgroup
% %\parbox{.44\linewidth}{
% %\def\arraystretch{1.1}%  1 is the default.
% \begin{tabular}{c|cccc}
%     \toprule
%     Argoverse & minADE$\,\downarrow$ & minFDE$\,\downarrow$ & MR$\,\downarrow$ & mAP$\,\uparrow$\\
%     \midrule
%      SEERNet & 0.69 & 1.24 & 0.09 & \todo{?} \\
%      ours (marginal) & \todo{?} & \todo{?} & \todo{?} & \todo{?} \\
%      ours (joint) & 0.70 & 1.20 & 0.12 & \todo{?} \\ 
%      \bottomrule
% \end{tabular}
% %}
% \egroup

% \vspace{0.2cm}
% \label{table:marginal-results}
% \caption{\textbf{Marginal predictive performance on self-driving car behavior prediction datasets.} Top: Waymo Open Motion Dataset \cite{ettinger2021large}, {\it standard} validation split. Bottom: Argoverse \cite{chang2019argoverse}. Reported are the minADE and minFDE for $k=6$ predictions \cite{alahi2016social,pellegrini2009you}, the Miss Rate (MR) \cite{chang2019argoverse} within 2 meters of the target, and the mean average precision (mAP) \cite{ettinger2021large}.}
% \end{table}

% \begin{table}[t]
% \centering
% \footnotesize
% \bgroup
% \def\arraystretch{1.1}%  1 is the default.
% %\parbox{.44\linewidth}{
% \begin{tabular}{c|ccc}
%     \toprule
%     Interactive & veh & ped & cyc \\
%     \midrule
%      baseline & 2.42 &  2.22 &3.02\\
%      ours (marginal) & {\bf 1.93} & {\bf 1.46} & {\bf 2.11} \\
%      ours (joint) & 2.46 & 1.92 & 2.73 \\ 
%      \bottomrule
% \end{tabular}
% %}
% %\\ \vspace{0.1cm}
% %\egroup
% %\vspace{0.3cm}
% \hspace{1.0cm}
% %\bgroup
% %\parbox{.44\linewidth}{
% %\def\arraystretch{1.1}%  1 is the default.
% \begin{tabular}{c|ccc}
%     \toprule
%     Standard & veh & ped & cyc \\
%     \midrule
%      baseline & 1.34 & 0.64 & 1.26\\
%      ours (marginal) & 1.70 & 0.94 & 1.66 \\
%      ours (joint) & 1.36 & 0.71 & 1.33 \\
%      \bottomrule
% \end{tabular}
% %}
% \egroup

% \vspace{0.2cm}
% \label{table:results-wmod}
% \caption{\textbf{Detailed predictive performance on Waymo Motion Open Dataset.} All numbers report minADE for \todo{$k=6$ predictions} \cite{alahi2016social,pellegrini2009you} at 8 seconds. Top: Interactive validation split. Bottom: Standard validation split.}
% \end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We train the \modelname on behavior prediction tasks from the Waymo Open Motion Dataset (\wmod) \cite{ettinger2021large} and the Argoverse dataset \cite{chang2019argoverse}. The \wmod dataset consists of 104,000 run segments (each 20 seconds in duration) over 1,750 km of unique roadways containing 7.64 million unique agent tracks. The Argoverse dataset consists of 324,000 run segments (each 5 seconds in duration) over 290 km of unique roadways containing 11.7 million unique agent tracks. We demonstrate that the resulting model achieves competitive or state of the art performance across these datasets. 

Most importantly, we demonstrate how the resulting joint future prediction model can employ masking strategies that map to various tasks, producing /emph{scene-consistent} predictions conditioned on behaviors or goals of specified agents.


\subsection{Scene Transformer provides high quality, consistent future predictions}
\label{sec:consistent}

The task of behavior prediction may be specified for the model by masking out the future positions of all agents in the scene. Conditional behavior prediction can be expressed by {\it not} masking out the future position of a specified agent, while masking out the future of all other agents.  We evaluate the quality of $k$ weighted trajectory hypotheses using a suite of standard evaluation metrics for behavior prediction in Table \ref{table:marginal-results} (See Methods).

{\bf Joint future predictions are consistent.} \todo{Some text.}

\begin{table}[t]
\centering
\footnotesize
\bgroup
\def\arraystretch{1.1}%  1 is the default.
%\parbox{.44\linewidth}{
\begin{tabular}{c|ccc}
    \toprule
    Interactive & veh & ped & cyc \\
    \midrule
     baseline & x &  x & x \\
     ours (marginal) & {\bf x} & {\bf x} & {\bf x} \\
     ours (joint) & x & x & x \\ 
     \bottomrule
\end{tabular}
%}
%\\ \vspace{0.1cm}
%\egroup
%\vspace{0.3cm}
\hspace{1.0cm}
%\bgroup
%\parbox{.44\linewidth}{
%\def\arraystretch{1.1}%  1 is the default.
\begin{tabular}{c|ccc}
    \toprule
    Standard & veh & ped & cyc \\
    \midrule
     baseline & x & x & x \\
     ours (marginal) & x & x & x \\
     ours (joint) & x & x & x \\
     \bottomrule
\end{tabular}
%}
\egroup

\vspace{0.2cm}
\label{table:collision_rates}
\caption{Agent-Agent collision rates of the most-likely prediction in \modelname compared to the baseline and the marginal \modelname in \wmod datasets.}
\end{table}


\begin{figure}[t]
\centering
\includegraphics[width=0.49\textwidth]{figures/Crab-Nebula.jpg} \hfill
\includegraphics[width=0.49\textwidth]{figures/Crab-Nebula.jpg} \hfill
\caption{Agent-Agent collision rates of the most-likely prediction as a function of x \todo{x=some slicing, like num valid agents, distance to traffic sign, etc} for \modelname, marginal \modelname and the baseline in \wmod Standard (left) and Interactive (right) datasets.}
\label{fig:collision_rate_slicing}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[width=0.49\textwidth]{figures/Crab-Nebula.jpg} \hfill
\includegraphics[width=0.49\textwidth]{figures/Crab-Nebula.jpg} \hfill
\caption{Example joint \modelname predictions (left) compared to the marginal \modelname (right) in a \textbf{lane merging} scenario.}
\label{fig:ex_lane_merge}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.49\textwidth]{figures/Crab-Nebula.jpg} \hfill
\includegraphics[width=0.49\textwidth]{figures/Crab-Nebula.jpg} \hfill
\caption{Example of most-likely predictions made by the marginal \modelname (right) compared to the joint \modelname (left). The marginal prediction results in a collision while the joint model supplies consistent, collision-free predictions.}
\label{fig:ex_marginal_collision}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.49\textwidth]{figures/Crab-Nebula.jpg} \hfill
\includegraphics[width=0.49\textwidth]{figures/Crab-Nebula.jpg} \hfill
\caption{Example of \textbf{homotopically different, yet consistent futures} predicted by \modelname (left) compared to marginal predictions (right)}
\label{fig:ex_homotopic}
\end{figure}



{\bf Joint future predictions capture complex agent interactions.} We demonstrate this in two parts.
First, our model achieves state of the art performance on behavior prediction benchmarks. 


\begin{table}[t]
\centering
\footnotesize
\bgroup
\def\arraystretch{1.1}%  1 is the default.
%\parbox{.44\linewidth}{
\begin{tabular}{c|ccc}
    \toprule
    Argoverse & minADE & MissRate & \todo{Others metrics} \\
    \midrule
     Method from leaderboard & x &  x & x \\
     ours (marginal) & {\bf x} & {\bf x} & {\bf x} \\
     ours (joint) & x & x & x \\ 
     \bottomrule
\end{tabular}
%}
%\\ \vspace{0.1cm}
%\egroup
%\vspace{0.3cm}
\hspace{1.0cm}
%\bgroup
%\parbox{.44\linewidth}{
%\def\arraystretch{1.1}%  1 is the default.
\begin{tabular}{c|ccc}
    \toprule
    WMOD & minADE & mAP & \todo{Others metrics} \\
    \midrule
     baseline & x & x & x \\
     ours (marginal) & x & x & x \\
     ours (joint) & x & x & x \\
     \bottomrule
\end{tabular}
%}
\egroup

\vspace{0.2cm}
\label{table:bp_metrics}
\caption{Argoverse and \wmod motion forecasting metrics \modelname compared to STOA methods.}
\end{table}


Next, our model achieves largest gains in scenarios that emphasize the interaction of agents in the environment.

\begin{table}[t]
\centering
\footnotesize
\bgroup
\def\arraystretch{1.1}%  1 is the default.
%\parbox{.44\linewidth}{
\begin{tabular}{c|ccc}
    \toprule
    WMOD Interactive & minADE & minFDE & mAP \\
    \midrule
     baseline & x &  x & x \\
     ours (marginal) & {\bf x} & {\bf x} & {\bf x} \\
     ours (joint) & x & x & x \\ 
     \bottomrule
\end{tabular}
\egroup
\vspace{0.2cm}
\label{table:bp_metrics}
\caption{\wmod Interactive dataset metrics of the \modelname compared to the baseline and the marginal Scene Transformer}
\end{table}


\begin{figure}[t]
\centering
\includegraphics[width=0.49\textwidth]{figures/Crab-Nebula.jpg} \hfill
\includegraphics[width=0.49\textwidth]{figures/Crab-Nebula.jpg} \hfill
\caption{minADE as a function of \todo{some slicing like num valid agents, distance to traffic sign, etc} for the \modelname and marginal \modelname in \wmod Interactive datasets.}
\label{fig:collision_rate_slicing}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Scene Transformer provides unified architecture for multi-task motion forecasting.}
\subsection{Scene Transformer as a unifying architecture for autonomous vehicle navigation}
\label{sec:gpm}

In Section \ref{sec:consistent}, we demonstrated that \modelname excels at behavior prediction. 
However, practical, safe autonomous vehicle navigation requires more than unconditional BP [].
For example...
Here we demonstrate that \modelname is a unifying end-to-end architecture that achieves  tasks critical in AV navigation through simple change of masking strategies. 
We demonstrate that \modelname performs BP, conditional BP [] and goal-directed motion planning using a {single trained model}.

{\bf Behavior prediction conditioned on an agent or AV trajectory.} \todo{Some text.}

\begin{figure}[t]
\centering
\includegraphics[width=0.49\textwidth]{figures/Crab-Nebula.jpg} \hfill
\includegraphics[width=0.49\textwidth]{figures/Crab-Nebula.jpg} \hfill
\caption{Cumulative distribution of minADE ratio between unconditional BP and BP conditioned on one of the two agents (left) or conditioned on the AV trajectory (right) for the WMOD Interactive dataset}
\label{fig:cpb_cum_minADE}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.49\textwidth]{figures/Crab-Nebula.jpg} \hfill
\includegraphics[width=0.49\textwidth]{figures/Crab-Nebula.jpg} \hfill
\caption{minADE ratio between unconditional BP and BP conditioned on one of the two agents (left) or conditioned on the AV trajectory (right) as a function of \todo{find a good slicing metric} for the WMOD Interactive dataset}
\label{fig:cpb_fn_minADE}
\end{figure}


{\bf Goal-directed motion planning.} \todo{Some text.}

\begin{figure}[t]
\centering
\includegraphics[width=0.49\textwidth]{figures/Crab-Nebula.jpg} \hfill
\includegraphics[width=0.49\textwidth]{figures/Crab-Nebula.jpg} \hfill
\caption{minADE ratio between unconditional BP and goal-directed AV motion planning for the WMOD Interactive dataset. Left: cumulative distribution. Right: as a function of \todo{find a good slicing metric}.}
\label{fig:planning_minADE}
\end{figure}

\begin{figure*}[t]
\centering
% “trim=1cm 2cm 3cm 4cm” trims (crops) from left, bottom, right and top by 1, 2, 3 and 4cm respectively. 
\includegraphics[width=0.325\textwidth, trim=0cm 7cm 0cm 2cm, clip=true]{figures/planning/10a90a1483a9c698-Original.png} 
\hfill
\includegraphics[width=0.325\textwidth, trim=0cm 7cm 0cm 2cm, clip=true]{figures/planning/10a90a1483a9c698-Joint.png}
\hfill
\includegraphics[width=0.325\textwidth, trim=0cm 1.5cm 0cm 0cm, clip=true]{figures/planning/10a90a1483a9c698-New-Target.png}

\includegraphics[width=0.325\textwidth, trim=0cm 7cm 0cm 2cm, clip=true]{figures/planning/10a90a1483a9c698-Original.png} 
\hfill
\includegraphics[width=0.325\textwidth, trim=0cm 7cm 0cm 2cm, clip=true]{figures/planning/10a90a1483a9c698-Joint.png}
\hfill
\includegraphics[width=0.325\textwidth, trim=0cm 1.5cm 0cm 0cm, clip=true]{figures/planning/10a90a1483a9c698-New-Target.png}

\includegraphics[width=0.325\textwidth, trim=0cm 7cm 0cm 2cm, clip=true]{figures/planning/10a90a1483a9c698-Original.png} 
\hfill
\includegraphics[width=0.325\textwidth, trim=0cm 7cm 0cm 2cm, clip=true]{figures/planning/10a90a1483a9c698-Joint.png}
\hfill
\includegraphics[width=0.325\textwidth, trim=0cm 1.5cm 0cm 0cm, clip=true]{figures/planning/10a90a1483a9c698-New-Target.png}

\caption{Example of goal-directed motion planning (middle, right)  compared to unconditional BP (left) in an intersection (top), lane change (middle), left/U-turning (bottom) scenario. The middle figure shows goal-directed planning when the ground truth end-point is used while the right figure uses an end-point specified by hand at inference time. \todo{Explain legend}}
% \caption{\textbf{Goal-directed planning navigates to desired location.} Rectangles indicate vehicles on the road. The autonomous vehicle (AV) is the light blue rectangle moving from right to left. Lines indicate the road graph (RG) colored by the type of lane marker. Circles indicate predicted trajectory for each agent. Left: Model is trained for BP only. AV attempts to take left turn but does not yield properly to the oncoming vehicle. Middle: Employ masking for goal-directed planning (Figure \ref{fig:model-architecture-diagram}, left). AV correctly yields to on-coming traffic before taking left turn. Correspondingly, oncoming traffic is predicted to progress further. Right: Same as previous, but the selected way point is to instead continue straight.}
\label{fig:planning_examples}
\end{figure*}


% {\bf Training on all masks are required to successfully use a model for all tasks.}
{\bf \modelname generalizes to all tasks.}
\todo{Some text.}

\begin{figure}[t]
\centering
\includegraphics[width=0.32\textwidth]{figures/Crab-Nebula.jpg}
\includegraphics[width=0.32\textwidth]{figures/Crab-Nebula.jpg}
\includegraphics[width=0.32\textwidth]{figures/Crab-Nebula.jpg}

\caption{minADE as a function of \todo{some slicing axis} for \modelname (blue) and \modelname trained on the unconditional BP (left), conditional BP (mid) and goal-directed motion planning (right) task only (red).}
\label{fig:ablation_masking_slice}
\end{figure}


\begin{table}[t]
\centering
\footnotesize
\bgroup
\def\arraystretch{1.1}%  1 is the default.
%\parbox{.44\linewidth}{
\begin{tabular}{c|ccc}
    \toprule
    WMOD Interactive minADE & BP & Conditional BP & Motion Planning \\
    \midrule
     \modelname & {\bf x} & {\bf x} & {\bf x} \\
     \modelname Single Task & x & x & x \\ 
     \bottomrule
\end{tabular}
\egroup
\vspace{0.2cm}
\label{table:ablation_masking}
\caption{minADE of \modelname for various tasks compared to \modelname trained with a single masking strategy matching the particular task (Single Task).}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Behavior prediction}

The task of behavior prediction may be specified for the model by masking out the future positions of agents in the scene. The task of conditional behavior prediction is distinct by {\it not} masking out the future position of the autonomous vehicle.

We evaluate the quality of $k$ weighted trajectory hypotheses using a suite of standard evaluation metrics for behavior prediction in Table \ref{table:marginal-results} (See Methods).

We find that the \modelname outperforms a strong baseline both when operating as a marginal and joint model. In Table \ref{table:marginal-results}, we find that the \modelname outperforms the strong baseline on marginal metrics for both the Waymo Open Motion Dataset standard split, and Argoverse. In Table \ref{table:results-wmod}, we find that the \modelname outperforms the strong baseline on joint metrics when evaluated on the interactive split of the Waymo Open Motion Dataset across all three class categories.

\subsection{Conditional behavior prediction}

\subsection{Goal-directed planning}



\subsection{Ablations and analysis}

\begin{enumerate}
    \item Waymo Open Motion Dataset and Argoverse
    \begin{enumerate}
        \item WOMD: Final numbers should be coming from Ben's runs with fixed padding + force time.
        \item Argoverse: As of 05/19, going to do a test submission on 5/19 to see if recent fixes with force time does it. Best result is with Bala's data aug.
    \end{enumerate}
    \item Analysis
    \begin{enumerate}
        \item Show how joint predictions are consistent (self-collision metrics exist, need to try to see if we should enable them; visualizations)
        \item If we talk about masking strategies, show CBP vs BP results (e.g. show the SDC, and show non-sdc BPs improve)
        \item Show slices of analysis across number of agents and geo.
    \end{enumerate}
    \item Ablations
    \begin{enumerate}
        \item Show performance difference with \# encoder / \# decoder layers. [*not* underway, may not be needed?]
        \item Architecture choices (how to layout the atten and x-atten layers) [*not* underway, may not be needed?]
    \end{enumerate}
\end{enumerate}


==> sections/old/results-very-very-old.tex <==
\section{Results}

\begin{table}[t]
\centering
\footnotesize
\bgroup
\def\arraystretch{1.1}%  1 is the default.
%\parbox{.44\linewidth}{
\begin{tabular}{c|cccc}
    \toprule
    %Waymo Open Motion &  minADE ($k$=$6$) & minFDE ($k$=$6$) & MissRate\,$@\,2m$ \\
    WOMD & minADE$\,\downarrow$ & minFDE$\,\downarrow$ & MR$\,\downarrow$ & mAP$\,\uparrow$\\
    \midrule
     SEERNet & 1.34 & - & 0.25 & \todo{?}\\
     ours (marginal) & 1.24 & 2.85 & 0.46 & \todo{?} \\
     ours (joint) & 1.54 & 3.75 & 0.49 & \todo{?} \\ 
     \bottomrule
\end{tabular}
%}
\\ \vspace{0.1cm}
%\egroup
%\vspace{0.3cm}
%\hfill
%\bgroup
%\parbox{.44\linewidth}{
%\def\arraystretch{1.1}%  1 is the default.
\begin{tabular}{c|cccc}
    \toprule
    Argoverse & minADE$\,\downarrow$ & minFDE$\,\downarrow$ & MR$\,\downarrow$ & mAP$\,\uparrow$\\
    \midrule
     SEERNet & 0.69 & 1.24 & 0.09 & \todo{?} \\
     ours (marginal) & \todo{?} & \todo{?} & \todo{?} & \todo{?} \\
     ours (joint) & 0.70 & 1.20 & 0.12 & \todo{?} \\ 
     \bottomrule
\end{tabular}
%}
\egroup

\vspace{0.2cm}
\label{table:marginal-results}
\caption{\textbf{Marginal predictive performance on self-driving car behavior prediction datasets.} Top: Waymo Open Motion Dataset \cite{ettinger2021large}, {\it standard} validation split. Bottom: Argoverse \cite{chang2019argoverse}. Reported are the minADE and minFDE for $k=6$ predictions \cite{alahi2016social,pellegrini2009you}, the Miss Rate (MR) \cite{chang2019argoverse} within 2 meters of the target, and the mean average precision (mAP) \cite{ettinger2021large}.}
\end{table}

\begin{table}[t]
\centering
\footnotesize
\bgroup
\def\arraystretch{1.1}%  1 is the default.
%\parbox{.44\linewidth}{
\begin{tabular}{c|ccc}
    \toprule
    Interactive & veh & ped & cyc \\
    \midrule
     baseline & 2.42 &  2.22 &3.02\\
     ours (marginal) & {\bf 1.93} & {\bf 1.46} & {\bf 2.11} \\
     ours (joint) & 2.46 & 1.92 & 2.73 \\ 
     \bottomrule
\end{tabular}
%}
%\\ \vspace{0.1cm}
%\egroup
%\vspace{0.3cm}
\hspace{1.0cm}
%\bgroup
%\parbox{.44\linewidth}{
%\def\arraystretch{1.1}%  1 is the default.
\begin{tabular}{c|ccc}
    \toprule
    Standard & veh & ped & cyc \\
    \midrule
     baseline & 1.34 & 0.64 & 1.26\\
     ours (marginal) & 1.70 & 0.94 & 1.66 \\
     ours (joint) & 1.36 & 0.71 & 1.33 \\
     \bottomrule
\end{tabular}
%}
\egroup

\vspace{0.2cm}
\label{table:results-wmod}
\caption{\textbf{Detailed predictive performance on Waymo Motion Open Dataset.} All numbers report minADE for \todo{$k=6$ predictions} \cite{alahi2016social,pellegrini2009you} at 8 seconds. Top: Interactive validation split. Bottom: Standard validation split.}
\end{table}


We train the scene transformer on the Waymo Open Motion Dataset \cite{ettinger2021large} and the Argoverse dataset \cite{chang2019argoverse} for behavior prediction tasks. Briefly, we demonstrate that the resulting model achieve competitive if not state of the art performance across these datasets. Importantly, we find that the resulting model makes joint predictions that are consistent suggesting that jointly modeling both other agents and the self-driving car behavior simultaneously results in sensible predictive representations. Finally, demonstrate a series of ablation studies to demonstrate the relative benefits of each part of the proposed architecture.

\subsection{Behavior prediction}

The task of behavior prediction may be specified for the model by masking out the future positions of agents in the scene. The task of conditional behavior prediction is distinct by {\it not} masking out the future position of the autonomous vehicle.

We evaluate the quality of $k$ weighted trajectory hypotheses using a suite of standard evaluation metrics for behavior prediction in Table \ref{table:marginal-results} (See Methods).

We find that the \modelname outperforms a strong baseline both when operating as a marginal and joint model. In Table \ref{table:marginal-results}, we find that the \modelname outperforms the strong baseline on marginal metrics for both the Waymo Open Motion Dataset standard split, and Argoverse. In Table \ref{table:results-wmod}, we find that the \modelname outperforms the strong baseline on joint metrics when evaluated on the interactive split of the Waymo Open Motion Dataset across all three class categories.

\subsection{Conditional behavior prediction}

\subsection{Goal-directed planning}

\begin{figure*}[t]
\centering
% “trim=1cm 2cm 3cm 4cm” trims (crops) from left, bottom, right and top by 1, 2, 3 and 4cm respectively. 
\includegraphics[width=0.325\textwidth, trim=0cm 7cm 0cm 2cm, clip=true]{figures/planning/10a90a1483a9c698-Original.png} 
\hfill
\includegraphics[width=0.325\textwidth, trim=0cm 7cm 0cm 2cm, clip=true]{figures/planning/10a90a1483a9c698-Joint.png}
\hfill
\includegraphics[width=0.325\textwidth, trim=0cm 1.5cm 0cm 0cm, clip=true]{figures/planning/10a90a1483a9c698-New-Target.png}
\caption{\textbf{Goal-directed planning navigates to desired location.} Rectangles indicate vehicles on the road. The autonomous vehicle (AV) is the light blue rectangle moving from right to left. Lines indicate the road graph (RG) colored by the type of lane marker. Circles indicate predicted trajectory for each agent. Left: Model is trained for BP only. AV attempts to take left turn but does not yield properly to the oncoming vehicle. Middle: Employ masking for goal-directed planning (Figure \ref{fig:model-architecture-diagram}, left). AV correctly yields to on-coming traffic before taking left turn. Correspondingly, oncoming traffic is predicted to progress further. Right: Same as previous, but the selected way point is to instead continue straight.}
\label{fig:planning-visualizations}
\end{figure*}

\subsection{Ablations and analysis}

\begin{enumerate}
    \item Waymo Open Motion Dataset and Argoverse
    \begin{enumerate}
        \item WOMD: Final numbers should be coming from Ben's runs with fixed padding + force time.
        \item Argoverse: As of 05/19, going to do a test submission on 5/19 to see if recent fixes with force time does it. Best result is with Bala's data aug.
    \end{enumerate}
    \item Analysis
    \begin{enumerate}
        \item Show how joint predictions are consistent (self-collision metrics exist, need to try to see if we should enable them; visualizations)
        \item If we talk about masking strategies, show CBP vs BP results (e.g. show the SDC, and show non-sdc BPs improve)
        \item Show slices of analysis across number of agents and geo.
    \end{enumerate}
    \item Ablations
    \begin{enumerate}
        \item Show performance difference with \# encoder / \# decoder layers. [*not* underway, may not be needed?]
        \item Architecture choices (how to layout the atten and x-atten layers) [*not* underway, may not be needed?]
    \end{enumerate}
\end{enumerate}


==> sections/old/womd-table-old.tex <==
% Some baseline numbers gathered from here:
% https://docs.google.com/document/d/1pKeoR0zzl21BoLjQ8fSe_nUt5hVSNueBTw1Yes5yPcA/edit
\begin{table}[t]
\centering
\footnotesize
\bgroup
\def\arraystretch{1.05}%  1 is the default.
\resizebox{\linewidth}{!}{
\begin{tabular}{cc|ccc|ccc|ccc|ccc}
    \toprule
    \multicolumn{2}{c|}{\multirow{2}{*}{{\bf Motion Prediction}}} & \multicolumn{3}{c|}{minADE$\,\downarrow$} & \multicolumn{3}{c|}{minFDE$\,\downarrow$} & \multicolumn{3}{c|}{MR$\,\downarrow$} & \multicolumn{3}{c}{mAP$\,\uparrow$} \\
    & & veh & ped & cyc & veh & ped & cyc & veh & ped & cyc & veh & ped & cyc\\ 
    \midrule
    {\it valid} & & & & & & & & & & & \\
     & LSTM baseline \cite{ettinger2021large} & 1.34 & 0.63 & 1.26 & 2.85 & 1.35 & 2.68 & 0.25 & 0.13 & 0.29 & 0.23 & 0.23 & \textbf{0.20} \\
     % From leaderboard submission
     & ours (marginal) & {\bf 1.17} & \textbf{0.59} & \textbf{1.15} & \textbf{2.51} & \textbf{1.26} & \textbf{2.44} & \textbf{0.20} & \textbf{0.12} & \textbf{0.24} & \textbf{0.26} & \textbf{0.27} & \textbf{0.20} \\
     & ours (marginal + NMS) & {\bf 1.23} & \textbf{0.75} & \textbf{1.25} & \textbf{2.64} & \textbf{1.68} & \textbf{2.68} & \textbf{0.20} & \textbf{0.24} & \textbf{0.27} & \textbf{0.33} & \textbf{0.26} & \textbf{0.26} \\
     % From leaderboard submission
     & ours (joint, bp-only) & 1.53 & 0.90 & 1.63 & 3.48 & 2.09 & 3.77 & 0.28 & 0.30 & 0.37 & 0.20 & 0.16 & 0.13\\
     % At 371.2K steps
     % https://tensorboard.corp.google.com/experiment/mldash:chauffeur:5237978701955273581/#scalars&regexInput=Dev&tagFilter=joint_metrics%2FVehicle_at_8s&_smoothingWeight=0
     & ours (joint, multi-task) & 1.56 & 0.89 & 1.60 & 3.56 & 2.06 & 3.68 & 0.29 & 0.29 & 0.37 & 0.19 & 0.15 & 0.15\\
     \midrule
    {\it test} & & & & & & & & & & & & \\
     & LSTM baseline \cite{ettinger2021large} & 1.34 & 0.64 & 1.29 & 2.83 & 1.35 & 2.68 & 0.24 & 0.13 & 0.29 & 0.24 & 0.22 & 0.19\\
     & ours (marginal) & \textbf{1.17} & \textbf{0.60} & \textbf{1.17} & \textbf{2.48} & \textbf{1.25} & \textbf{2.43} & \textbf{0.19} & \textbf{0.12} & \textbf{0.22} & \textbf{0.27} & \textbf{0.23} & \textbf{0.20}\\
     & ours (marginal + NMS) & \textbf{1.22} & \textbf{0.76} & \textbf{1.27} & \textbf{2.61} & \textbf{1.68} & \textbf{2.69} & \textbf{0.20} & \textbf{0.23} & \textbf{0.27} & \textbf{0.33} & \textbf{0.27} & \textbf{0.25}\\
     & ours (joint, bp-only) & 1.52 & 0.91 & 1.61 & 3.43 & 2.09 & 3.68 & 0.28 & 0.30 & 0.37 & 0.19 & 0.16 & 0.19\\
     & ours (joint, multi-task) & 1.55 & 0.91 & 1.64 & 3.50 & 2.08 & 3.75 & 0.28 & 0.29 & 0.38 & 0.19 & 0.16 & 0.19\\
     \bottomrule
\end{tabular}}
\egroup
\\ \vspace{0.2cm}
\bgroup
\def\arraystretch{1.05}%  1 is the default.
\resizebox{\linewidth}{!}{
\begin{tabular}{cc|ccc|ccc|ccc|ccc}
    \toprule
    \multicolumn{2}{c|}{\multirow{2}{*}{{\bf Interaction Prediction}}} & \multicolumn{3}{c|}{minSADE$\,\downarrow$} & \multicolumn{3}{c|}{minSFDE$\,\downarrow$} & \multicolumn{3}{c|}{SMR$\,\downarrow$} & \multicolumn{3}{c}{mAP$\,\uparrow$}\\
    & & veh & ped & cyc & veh & ped & cyc & veh & ped & cyc & veh & ped & cyc\\ 
    \midrule
    {\it valid} & & & & & & & & & & &\\
     & LSTM baseline \cite{ettinger2021large} & 2.42 & 2.73 & 3.16 & 6.07 & 4.20 & 6.46 & 0.66 & 1.00 & 0.83 & 0.07 & \textbf{0.06} & 0.02 \\
     % From leaderboard submission
     & ours (marginal) & 2.04 & 1.62 & 2.28 & 4.94 & 3.81 & 5.67 & 0.54 & 0.63 & 0.72 & \textbf{0.11} & 0.05 & 0.03 \\
     % From leaderboard submission
     & ours (joint, bp-only) & \textbf{1.72} & \textbf{1.38} & 1.96 & \textbf{3.98} & \textbf{3.11} & 4.75 & \textbf{0.49} & \textbf{0.60} & 0.73 & \textbf{0.11} & 0.05 & 0.03  \\
     % At 371.2K steps
     % https://tensorboard.corp.google.com/experiment/mldash:chauffeur:5237978701955273581/#scalars&regexInput=Dev&tagFilter=joint_metrics%2FVehicle_at_8s&_smoothingWeight=0
     & ours (joint, multi-task) & \textbf{1.72} & 1.39 & \textbf{1.94} & 3.99 & 3.15 & \textbf{4.69} & \textbf{0.49} & 0.62 & \textbf{0.71} & \textbf{0.11} & \textbf{0.06} & \textbf{0.04} \\     
     \midrule
    {\it test} & & & & & & & & & & & \\
     & LSTM baseline \cite{ettinger2021large} & 2.46 & 2.47 & 2.96 & 6.22 & 4.30 & 6.26 & 0.67 & 0.89 & 0.89 & 0.06 & 0.03 & 0.03\\
     % At 857.6K steps
     & ours (marginal) & 2.08 & 1.62 & 2.24 & 5.04 & 3.87 & 5.41 & 0.55 & 0.64 & 0.73 & 0.08 & \textbf{0.05} & 0.03 \\
     & ours (joint, bp-only) & 1.76 & \textbf{1.38} & \textbf{1.95} & 4.08 & \textbf{3.19} & \textbf{4.65} & \textbf{0.50} & \textbf{0.62} & \textbf{0.70} & 0.10 & \textbf{0.05} & \textbf{0.04}\\
     & ours (joint, multi-task) & \textbf{1.74} & 1.41 & \textbf{1.95} & \textbf{4.06} & 3.26 & 4.68 & \textbf{0.50} & 0.64 & 0.71 & \textbf{0.13} & 0.04 & 0.03\\
     \bottomrule
\end{tabular}}
\egroup
\vspace{0.2cm}
\label{table:wmod-results}
\caption{\textbf{Predictive performance for $t=8$ seconds on Waymo Open Motion Dataset trajectory prediction} \cite{ettinger2021large}. Top: Marginal predictive performance based on the {\it standard} splits of the validation and test datasets evaluated with traditional \textit{marginal metrics}. Bottom: Joint predictive performance based on the {\it interactive} splits of the validation and test datasets evaluated with scene level \textit{joint metrics}. Reported are the min(S)ADE, min(S)FDE for $k=6$ predictions \cite{alahi2016social,pellegrini2009you}, and the Miss Rate (MR) \cite{chang2019argoverse} within 2 meters of the target, where S indicates a scene-level joint metric \cite{ettinger2021large}. See Appendix for $t=3$ and $t=5$ seconds.}
\vspace{-0.6cm}
\end{table}
